Individual and Collective Performance Deteriorate in a New Team: A Case Study of CS:GO Tournaments

How does the team formation relates to team performance in professional video game playing? This study examined one aspect of group dynamics - team switching - and aims to answer how changing a team affects individual and collective performance in eSports tournaments. In this study we test the hypothesis that switching teams can be detrimental to individual and team performance both in short term and in a long run. We collected data from professional tournaments of a popular first-person shooter game {\itshape Counter-Strike: Global Offensive (CS:GO)} and perform two natural experiments. We found that the player's performance was inversely correlated with the number of teams a player had joined. After a player switched to a new team, both the individual and the collective performance dropped initially, and then slowly recovered. The findings in this study can provide insights for understanding group dynamics in eSports team play and eventually emphasize the importance of team cohesion in facilitating team collaboration, coordination, and knowledge sharing in teamwork in general.

==> csgo_arxiv/table_mod2inditeam.tex <==
\begin{tabular}{r l l l l l l l l l l} 
    \toprule
    \textbf{}&\multicolumn{2}{c}{\# Kills} 
    &\multicolumn{2}{c}{\# Head shots}
    &\multicolumn{2}{c}{\# Assists} 
    &\multicolumn{2}{c}{\# Flash assists}
    &\multicolumn{2}{c}{\# Deaths}\\
    &\multicolumn{1}{c}{Player}
    &\multicolumn{1}{c}{Team} 
    &\multicolumn{1}{c}{Player} 
    &\multicolumn{1}{c}{Team} 
    &\multicolumn{1}{c}{Player} 
    &\multicolumn{1}{c}{Team} 
    &\multicolumn{1}{c}{Player} 
    &\multicolumn{1}{c}{Team} 
    &\multicolumn{1}{c}{Player} 
    &\multicolumn{1}{c}{Team} \\
    \midrule
    Intercept 
    &11.44 (0.13)$^{***}$ 
    &13.76 (0.19)$^{***}$
    &\ 3.26 (0.05)$^{***}$ &\ 4.51 (0.01)$^{***}$
    &\ 2.22 (0.03)$^{***}$ &\ 2.01 (0.04)$^{***}$
    &\ 0.18 (0.02)$^{***}$ &\ 0.23 (0.01)$^{***}$
    &\ 13.76 (0.13)$^{***}$ &\ 14.63 (0.21)$^{***}$\\
    Prior performance 
    &\ 0.33 (0.01)$^{***}$ &\ 0.20 (0.01)$^{***}$
    &\ 0.58 (0.01)$^{***}$ &\ 0.41 (0.01)$^{***}$
    &\ 0.37 (0.01)$^{***}$ &\ 0.47 (0.01)$^{***}$
    &\ 0.65 (0.01)$^{***}$ &\ 0.69 (0.01)$^{***}$
    &\ 0.24 (0.01)$^{***}$ &\ 0.19 (0.01)$^{***}$\\
    Match index
    &\ 0.09 (0.02)$^{***}$ &\ 0.12 (0.02)$^{***}$
    &\ 0.03 (0.01)$^{***}$ &\ 0.04 (0.01)$^{***}$
    &\ 0.09 (0.01)$^{***}$ &\ 0.05 (0.01)$^{***}$
    &\ 0.04 (0.004)$^{***}$ &\ 0.02 (0.003)$^{***}$
    &-0.02 (0.01)$^{*}$ &-0.18 (0.02)$^{***}$\\
    Treatment 
    &-0.24 (0.10)$^{**}$ &-0.51 (0.10)$^{***}$
    &\ 0.11 (0.05)$^{*}$ &-0.14 (0.05)$^{**}$
    &\ 0.15 (0.03)$^{***}$ &-0.11 (0.03)$^{***}$
    &\ 0.06 (0.02)$^{*}$ &-0.03 (0.02)
    &\ 0.22 (0.01)$^{**}$ &\ 0.42 (0.01)$^{***}$\\
    Match index $\times$ 
    &\ 0.02 (0.02) &\ 0.11 (0.03)$^{***}$
    &-0.04 (0.01)$^{**}$ &\ 0.03 (0.01)$^{**}$
    &-0.03 (0.01)$^{**}$ &\ 0.02 (0.01)$^{**}$
    &-0.01 (0.01) &\ 0.01 (0.004)
    &-0.06 (0.02)$^{***}$ &-0.08 (0.03)$^{**}$\\
    \    Treatment \\
    \midrule
    Random effect
    &1.24 &0.29
    &0.56 &0.18
    &0.15 &0.09
    &0.03 &0.01
    &0.42 &0.31\\
    Log-likelihood
    &-1,426,971 &-315,608
    &-1,183,122 &-233,738
    &-993,745 &-190,654
    &-384,964 &-65,224
    &-1,305,106 &-317,353\\
    N
    &438,080 &108,842
    &438,080 &108,842
    &438,080 &108,842
    &246,986 &67,081
    &438,080 &108,842\\
    \midrule
    \textbf{}&\multicolumn{2}{c}{KAST} 
    &\multicolumn{2}{c}{K-D Diff}
    &\multicolumn{2}{c}{FK Diff} 
    &\multicolumn{2}{c}{ADR}
    &\multicolumn{2}{c}{Rating}\\
    &\multicolumn{1}{c}{Individual}
    &\multicolumn{1}{c}{Teammate} 
    &\multicolumn{1}{c}{Individual} 
    &\multicolumn{1}{c}{Teammate} 
    &\multicolumn{1}{c}{Individual} 
    &\multicolumn{1}{c}{Teammate} 
    &\multicolumn{1}{c}{Individual} 
    &\multicolumn{1}{c}{Teammate} 
    &\multicolumn{1}{c}{Individual} 
    &\multicolumn{1}{c}{Teammate} \\
    \midrule
    Intercept
    &51.55 (0.49)$^{***}$ &47.65 (0.78)$^{***}$
    &-0.45 (0.07)$^{***}$ &-0.57 (0.07)$^{***}$
    &-0.12 (0.02)$^{***}$ &-0.13 (0.02)$^{***}$
    &48.36 (0.55)$^{***}$ &49.51 (0.83)$^{***}$
    &\ 0.627 (0.007)$^{***}$ &\ 0.663 (0.011)$^{***}$\\
    Prior performance
    &\ 0.24 (0.02)$^{***}$ &\ 0.29 (0.01)$^{***}$
    &\ 0.38 (0.01)$^{***}$ &\ 0.33 (0.01)$^{***}$
    &\ 0.26 (0.01)$^{***}$ &\ 0.22 (0.01)$^{***}$
    &\ 0.36 (0.01)$^{***}$ &\ 0.33 (0.01)$^{***}$
    &\ 0.37 (0.007)$^{***}$ &\ 0.38 (0.010)$^{***}$\\
    Match index
    &\ 0.21 (0.04)$^{***}$ &\ 0.28 (0.05)$^{***}$
    &\ 0.07 (0.02)$^{***}$ &\ 0.13 (0.02)$^{***}$
    &\ 0.02 (0.01)$^{***}$ &\ 0.03 (0.005)$^{***}$
    &-0.06 (0.06) &\ 0.13 (0.05)$^{**}$
    &\ 0.006 (0.001)$^{***}$ &\ 0.007 (0.001)$^{***}$\\
    Treatment 
    &-0.61 (0.21)$^{**}$ &-1.55 (0.26)$^{***}$
    &-0.30 (0.10)$^{**}$ &-0.77 (0.11)$^{***}$
    &-0.13 (0.03)$^{***}$ &-0.16 (0.03)$^{***}$
    &-1.04 (0.32)$^{**}$ &-1.32 (0.25)$^{***}$
    &-0.007 (0.001) &-0.038 (0.006)$^{***}$\\
    Match index $\times$ 
    &\ 0.14 (0.05)$^{**}$ &\ 0.32 (0.07)$^{***}$
    &\ 0.05 (0.02) &\ 0.16 (0.03)$^{***}$
    &\ 0.03 (0.01)$^{**}$ &\ 0.03 (0.01)$^{***}$
    &\ 0.12 (0.08) &\ 0.27 (0.07)$^{***}$
    &\ 0.001 (0.001) &\ 0.008 (0.002)$^{***}$\\
    \    Treatment \\
    \midrule
    Random effects
    &3.67 &3.96
    &1.69 &0.96
    &0.12 &0.03
    &14.86 &3.66
    &0.004 &0.003\\
    Log-likelihood
    &-1,303,831 &-325,528
    &-1,479,762 &-327,440
    &-1,007,923 &-175,981
    &-1,437,002 &-322,907
    &-151,489 &-3,544\\
    N
    &331,774 &87,893
    &438,080 &108,842
    &438,080 &108,842
    &331,662 &87,876
    &438,080 &108,842\\
    \bottomrule
    \end{tabular}
